Gyrokinetic moment-based simulations of the Dimits shift

We present a convergence study of the gyromoment (GM) approach, which is based on projecting the gyrokinetic distribution function onto a Hermite-Laguerre polynomial basis, focused on the cyclone base case (CBC) (Lin et al. 1999) and Dimits shift (Dimits et al. 2000) as benchmarks. We report that the GM approach converges more rapidly in capturing the nonlinear dynamics of the CBC than the continuum GENE code (Jenko et al. 2000) when comparing the number of points representing the velocity space. Increasing the velocity dissipation improves the convergence properties of the GM approach, albeit yielding a slightly larger saturated heat flux. By varying the temperature equilibrium gradient, we show that GM approach successfully reproduces the Dimits shift (Dimits et al. 2000) and effectively captures its width, which is in contrast to the gyrofluid framework. In the collisional regime, the convergence properties of the GM approach improve and a good agreement with previous global PIC results on transport is obtained (Lin et al. 1999). Finally, we report that the choice of collision model has a minimal impact both on the ITG growth rate and on the nonlinear saturated heat flux, at tokamak-relevant collisionality.

==> AX_side_tests.tex <==
\section{Side notes and tests}

Here are some side tests we did and their conclusion.
Should we put them in the paper?

\begin{itemize}
    \item We compared simulations between single and double precision representation and did not observe any significant change in the nonlinear transport nor the ITG instability spectrum.
    We note only that it is not possible to run a large Laguerre polynomial basis simulation ($J \gtrsim 20$) with single precision due to the kernel function computation that works with very large numbers.
    Overall, a $\sim 50\%$ speedup is observed for single precision runs.

    \item We run every nonlinear simulation with a $n=0$ truncation in the Hermite-Laguerre projection of the nonlinear term.

    \item For larger collision values, the size of the box must be increased to avoid box size effects

    \item The GK linear collision operators are capped at $k_\perp = 1$ to avoid high frequencies that forces a large reduction the time step size.
    We varied this value without noticing changes.

    \item Initialization with noise instead of a smooth Gaussian/Jacobian power is very unstable.

    \item The staggered grid can be replaced by simples numerical diffusion in $z$.

    \item The application of the collision matrix is dominating the computation cost.
    We compare the share of computational cost used for the collision term in our standard collisional spatial resolution, i.e. $N_{x} \times N_{y} \times N_z = 192\times 96 \times 24$, for different polynomial sets, $(4,2)$, $(8,4)$ and $(16,8)$.
    The computation of the DGGK operator (not a collision matrix) takes around $4.3\%$ of the total computational cost for the three polynomial sets.
    For the SGGK collision matrix, the computation time share of the collision term evaluation is $30\%$ for $(4,2)$, $60\%$ for $(8,4)$ and $80\%$ for $(16,8)$.
    This is related to the fact that applying the collision matrix is an operation of cost $O(P^2J^2)$ whereas the other operations are all linear in the number of polynomials.
    
\end{itemize}


==> backup.tex <==
% \begin{align}
%     &\ddt N_a^{pj}+ \frac{\tau_a}{q_a} i k_y \squareparenthesis{\sqrt{(p+1)(p+2)} n_a^{p+2,j} + (2p+1)n_a^{p,j} + \sqrt{p(p-1)}n_a^{p-2,j}}\nonumber\\
%     %
%     &+ \frac{\tau_a}{q_a} i k_y \squareparenthesis{(2j+1)n_a^{pj} - (j+1)n_a^{p,j+1}-jn_a^{p,j-1}}\nonumber\\
%     %
%     &-\kappa_N ik_y\phi\squareparenthesis{\roundparenthesis{1-\frac{3}{2}\eta}\kernel_j\delta_{p}^0 + \eta\kernel_j\roundparenthesis{\frac{1}{2}\delta_p^0 + \frac{1}{\sqrt{2}}\delta_p^2} + \eta([2j+1]\kernel_j-[j+1]\kernel_{j+1}-j\kernel_{j-1})\delta_p^0} \nonumber\\
%     &=\sum_{ab}C_{ab}^{pj}+\squareparenthesis{\sum_{n=0}^{\infty}\roundparenthesis{ik_x\kernel_n\phi}*\roundparenthesis{ik_y\sum_{s=0}^{n+j}d_{njs}N_a^{ps}} - \roundparenthesis{ik_y\kernel_n\phi}*\roundparenthesis{ik_x\sum_{s=0}^{n+j}d_{njs}N_a^{ps}}}
%     \label{eq:moment_gyboeq_nondim_nonadiab}.
% \end{align}
% We use, in equation \eqref{eq:moment_gyboeq_nondim_nonadiab}, the magnetic gradient length $L_{\textrm{ref}}=L_B$ as reference length and the sound Larmor radius for the typical fluctuation scale, i.e. $k_{x,y,\textrm{ref}}=1/\rho_s= \Omega_i/c_s$ where $c_s=\sqrt{T_e/m_i}$ is the sound speed and $\Omega_i=\sqrt{eB/m_i}$ the ion cyclotron frequency. 
% We also introduce the dimensionless temperature and mass ratios, i.e. $\tau_a=T_a/T_i$ and $\sigma_a=\sqrt{m_a/m_i}$, respectively.

==> dimensions.tex <==
\topmargin=-0.45in      %
%\evensidemargin=0in     %
\oddsidemargin=-0.1in      %
\textwidth=6.8in        %
\textheight=9.2in       %
%\headsep=0.25in         %
\headheight=30.9pt

==> equations/moment_hierarchy_full.tex <==
\begin{align}
    &\ddt N_a^{pj}+\sum_{n=0}^{\infty}\curlyparenthesis{\kernel_n\phi,\sum_{s=0}^{n+j}d_{njs} N_a^{ps}}
    %
    \nonumber\\&
    %
    + \frac{\tau_a}{q_a} \mathcal C_{k_x k_y} \squareparenthesis{\sqrt{(p+1)(p+2)} n_a^{p+2,j} + (2p+1)n_a^{p,j} + \sqrt{p(p-1)}n_a^{p-2,j}}
    %
    \nonumber\\&
    %
    + \frac{\tau_a}{q_a} \mathcal C_{k_x k_y} \squareparenthesis{(2j+1)n_a^{pj} - (j+1)n_a^{p,j+1}-jn_a^{p,j-1}}
    %
    \nonumber\\&
    %
    +ik_y\phi\squareparenthesis{\kNa\kernel_j\delta_{p}^0 +\kTa \roundparenthesis{\kernel_j\roundparenthesis{\frac{1}{\sqrt{2}}\delta_p^2 -\delta_p^0}+ ([2j+1]\kernel_j-[j+1]\kernel_{j+1}-j\kernel_{j-1})\delta_p^0}}
    %
    \nonumber\\&
    %
    + \frac{\hat B^{-1}}{J_{xyz}} \frac{\sqrt{\tau_a}}{\sigma_a}\left\{\squareparenthesis{\sqrt{p+1}\ddz n_a^{p+1,j} + \sqrt{p} \ddz n_a^{p-1,j}}\right.
    %
    \nonumber\\&
    %
    \quad- \ddz\ln B \left[(j+1)(\sqrt{p+1} n_a^{p+1,j} + \sqrt{p} n_a^{p-1,j})\right.
    %
    % \nonumber\\&
    %
    % \left.-j(\sqrt{p+1} n_a^{p+1,j-1} + \sqrt{p} n_a^{p-1,j-1})\right]
    \left.-(2j-1)(\sqrt{p+1} n_a^{p+1,j-1} + \sqrt{p} n_a^{p-1,j-1})\right]
    %
    \nonumber\\&
    %
    % \quad\left. -\ddz\ln B\sqrt{p}\squareparenthesis{(2j+1)N_a^{p-1,j} - jN_a^{p-1,j-1}-(j+1)N_a^{p-1,j+1}}\right\}=C_{a}^{pj}
    \quad\left. +\ddz\ln B\sqrt{p}\squareparenthesis{(2j+1)N_a^{p-1,j} - jN_a^{p-1,j-1}-(j+1)N_a^{p-1,j+1}}\right\}=C_{a}^{pj}
    \label{eq:moments_hier_curvlin}
\end{align}

==> nonlin_term.tex <==
\subsection{Moments equation right-hand-side : nonlinear term}
In the moments formulation \eqref{eq:moment_gyboeq_nondim}, we ended up with a nonlinear term that has to be treated carefully, i.e.
\begin{align}
    S_a^{pj} :&= ||\mathcal{F}[\grad \dphi \times \grad \dga ]||_a^{pj} \nonumber\\
    &= \epsilon^{-1}\int\sum_{n=0}^{\infty} \bvec\cdot\roundparenthesis{\phi[\bm k']\kernel_n[b']\bm k'\times (\bm k - \bm k')\sum_{s=0}^{n+j}d_{njs}N_a^{ps}[\bm k -\bm k']}d\bm k'
\end{align}
The high order $\epsilon^{-1}$ factor in front can be removed by normalizing our perturbation fields by $\epsilon$ so that $\phi \times N_a^{pj}\sim \epsilon^2$ and
resulting into a $\epsilon^1$ factor that simplifies with the linear terms ones.
Once this small normalization done, the nonlinear term can be written in a more explicit format as
\begin{align}
    &\int \sum_{n=0}^{\infty}(k_z'-k_r')\phitilde[\bm k']\kernel_n[b']((k_z-k_z')-(k_r-k_r'))\sum_{s=0}^{n+j}d_{njs}N_a^{ps}[\bm k -\bm k']d\bm k'\nonumber\\
    %
    &=\sum_{n=0}^{\infty}\int \underbrace{(k_z'-k_r')\phitilde[\bm k']\kernel_n[b']}_{\Phi_n[\bm k']}%
    \cdot\underbrace{(\Delta k_z'-\Delta k_r')\Sigma_{s=0}^{n+j}d_{njs}N_a^{ps}[\Delta\bm k']}_{\Gamma_{an}^{pj}[\bm k-\bm k']}d\bm k'\nonumber\\
    %
    &=\sum_{n=0}^{\infty} (\Phi_n *  \Gamma_{an}^{pj})[\bm k] %
    =\sum_{n=0}^{\infty}\mathcal{F}\roundparenthesis{\mathcal{F}^{-1}\squareparenthesis{\Phi_n} \cdot \mathcal{F}^{-1}\squareparenthesis{\Gamma_{an}^{pj}}}%
    =\mathcal{F}\roundparenthesis{\sum_{n=0}^{\infty}\mathcal{F}^{-1}\squareparenthesis{\Phi_n} \cdot \mathcal{F}^{-1}\squareparenthesis{\Gamma_{an}^{pj}}}
    \label{eq:2nd_term_convolution_th}
\end{align}
This notation points out the possibility to use Fourier transform instead of integrals thanks of the convolution theorem $\mathcal{F}[f * g] = \mathcal{F}[f] \cdot \mathcal{F}[g]$. It is worth noting that this formulation may be more computationally intense than the one in GS2 (\cite{Highcock2012}) where the derivatives were simply replaced by an inverse Fourier transform, i.e.
\begin{equation}
    \partial_z\phi \partial_r g = \mathcal{F}^{-1}[ik_z J_0 \phi] \cdot \mathcal{F}^{-1}[i k_r g].
\end{equation}
In our case, the Bessel function was projected on the Hermite-Laguerre basis which lead to the sum of kernel functions $\kernel_n$. 
\\
One can design a process that allows us to obtain the non-linear term $S_a^{pj}$ at a given wave vector $\bm k$ by using discrete fast Fourier transform (FFT), avoiding the convolution integral.
FFT consists in a transformation of a signal $\{f_j\}_{j=0}^{N-1}$ to a frequency spectrum $\{F_k\}_{k=0}^{N-1}$ as\footnote{The following development has inspired by \textit{How Important is Dealiasing for Turbulence Simulations?} from John C. Bowman, University of Alberta, September 30, 2014.}

\begin{equation}
    \mathrm{FFT}[f]_k = F_k = \frac{1}{N}\sum_{j=0}^{N-1}(\zeta_N)^{-kj}f_j
\end{equation}

and the inverse transform

\begin{equation}
    \mathrm{FFT}^{-1}[F]_j = f_j = \sum_{k=0}^{N-1}(\zeta_N)^{jk}F_k
\end{equation}
where the weights are defined $\zeta_N=e^{-2\pi i/N}$ and fulfill the relation
\begin{equation}
    \sum_{j=0}^{N-1}(\zeta_N)^{lj} = 
    \begin{cases}
    N& \text{if $l=sN$ for $s\in\mathbb{Z}$}\\
    0              & \text{otherwise}
    \end{cases}
    \label{eq:zeta_id}
\end{equation}
Thus in a one dimensional discrete case, our convolution term transformed in a real space product can be written as
\begin{align}
    (F*G)_k = \textrm{FFT}[f\cdot g]_k &=\sum_{j=0}^{N-1} f_{j} g_{j}(\zeta_N)^{-kj}\nonumber\\
    %
    &=\sum_{j=0}^{N-1} (\zeta_N)^{-kj} \sum_{l=0}^{N-1}(\zeta_N)^{jl}F_l \sum_{m=0}^{N-1}(\zeta_N)^{jm}G_m \nonumber\\
    & \sum_{l=0}^{N-1} F_l \sum_{m=0}^{N-1} G_m \sum_{j=0}^{N-1} (\zeta_N)^{(l+m-k)j}\nonumber\\
    %
    \rvert_\eqref{eq:zeta_id}&=N\sum_s\sum_{l=0}^{N-1}F_l G_{k-l+sN}
    \label{eq:aliasing}
\end{align}
Thus, it is important to notice that that in the discrete case, the convolution theorem lead to additional terms called aliases, corresponding to each $G_{k-l+sN}$ where $s\neq 0$. These terms will introduce unwanted errors in the computation of the linear term and must be removed by ensuring that $G_{k-l+sN} = 0$ whenever $s\neq 0$.\\
Practically, if $F_n$ and $G_n$ are nonzero only up to $n\leq M$, a non aliased convolution can be set up by extending our signal to $N \geq 2M -1$ since it will cancel each terms for $k-l+sN\geq M$.


In two dimensions the discrete convolution is derived in Appendix \ref{appendix:2D_aliasing} and is a simple extension from the 1D case leading to the anti-aliasing condition
\begin{equation*}
    G_{k_r - l_r + s_r N_r,k_z - l_z + s_z N_z} = 0 \quad \forall s_r,s_z\neq 0.
\end{equation*}
In conclusion, one can dealiase completely our 2D signal by zero padding the discretized expression of $\Phi_{an}$ and $\Pi_{an}^{pj}$ found in \eqref{eq:2nd_term_convolution_th}.
One can summarize the work done in this chapter by the following algorithm

\begin{algorithm}
\caption{Nonlinear term computation}
\label{alg:conv_FFT}
\begin{algorithmic}[ht]
    \STATE $\{S_a^{pj}\}_{k_r,k_z=0}^{M_r,M_z} \gets 0$
    \FORALL{$n=0,J_{max,a}-j$}
    \STATE $\{F_{k_r,k_z}\}_{k_r,k_z=0}^{N_r,N_z} \gets \{(k_z-k_r)\phitilde[\bm k]\kernel_n[b_a]\}_{k_r,k_z=0}^{N_r,N_z}$
    \STATE
    \STATE $\{G_{k_r,k_z}\}_{k_r,k_z=0}^{N_r,N_z} \gets \{(k_z-k_r)\sum_{s=0}^{n+j}d_{njs}N_a^{ps}[\bm k]\}_{k_r,k_z=0}^{N_r,N_z}$
    \STATE
    \STATE$\{F_{k_r,k_z}\}_{k_r,k_z=0}^{M_r,M_z} \gets $ zero padding$\roundparenthesis{\{F_{k_r,k_z}\}_{k_r,k_z=0}^{N_r,N_z},\, M = 2N -1}$
    \STATE
    \STATE$\{G_{k_r,k_z}\}_{k_r,k_z=0}^{M_r,M_z} \gets $ zero padding$\roundparenthesis{\{G_{k_r,k_z}\}_{k_r,k_z=0}^{N_r,N_z},\, M = 2N -1}$
    \STATE
    \STATE $\{f_{r,z}\}_{k_r,k_z=0}^{M_r,M_z} \gets \textrm{FFT}^{-1}\squareparenthesis{\{F_{k_r,k_z}\}_{k_r,k_z=0}^{M_r,M_z}}$
    \STATE
    \STATE $\{g_{r,z}\}_{k_r,k_z=0}^{M_r,M_z} \gets \textrm{FFT}^{-1}\squareparenthesis{\{G_{k_r,k_z}\}_{k_r,k_z=0}^{M_r,M_z}}$
    \STATE
    \STATE $\{S_a^{pj}\}_{k_r,k_z=0}^{M_r,M_z} \gets \{S_a^{pj}\}_{k_r,k_z=0}^{M_r,M_z} + \{f_{r,z}\cdot g_{r,z}\}_{k_r,k_z=0}^{M_r,M_z}$
    \ENDFOR
    \RETURN $\textrm{FFT}\squareparenthesis{\{S_a^{pj}\}_{k_r,k_z=0}^{N_r,N_z}}$
\end{algorithmic}
\end{algorithm}

This algorithm does not show however the truncation that is needed in order to compute the term $G$ since the $N_a^{ps}$ are defined up to $s = J_{max,a}$. Practically, it is achieved by setting the upper bound of the sum over $s$ to $min(J_{max,a},n+j)$, i.e.
$$
G = (k_z-k_r)\sum_{s=0}^{n+j}d_{njs}N_a^{ps}[\bm k] \approx (k_z-k_r)\sum_{s=0}^{min(n+j,J_{max,a})}d_{njs}N_a^{ps}[\bm k]
$$

==> tables_and_graphics/32_CBC_linear_transp_estimate.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/32_CBC_linear_transp_estimate.eps}
    \vspace{-0.5cm}
    \caption{Comparison of the CBC linear transport spectrum estimates, $\gamma/k_y^2$, between the results obtained by the GM approach (a), the GENE code (b) and  \cite{Dimits2000ComparisonsSimulations}. 
    We present results from different polynomial sets $(P,J)$ for the GM approach and velocity grid resolutions $N_{v\parallel}\times N_\mu$ for GENE.
    We also report GENE results with halved velocity domain $L_{\vpar}\times L_\mu=4.5\times 1.5$ (dashed lines).}
    \label{fig:32_CBC_linear_transp_estimate}
\end{figure}

==> tables_and_graphics/old_32_CBC_nonlinear_convergence.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/32_CBC_nonlinear_convergence.eps}
    \vspace{-0.5cm}
    \caption{(a) Time traces of the heat flux for the CBC, comparison between the gyromoment approach, GENE and the results of \cite{Dimits2000ComparisonsSimulations} for various velocity resolutions. The legend denotes the different polynomial sets $(P,J)$ used by the GM approach as well as the number of points in the GENE velocity grid $N_{\vpar}\times N_\mu$.
    (b) Moments energy spectrum $E(p,j)=\sum_{k_x,k_y,z}|N_a^{pj}(k_x,k_y,z)|$ of the CBC, time averaged for the second half of the time traces presented in (a).}
    \label{fig:32_CBC_nonlinear_convergence}
\end{figure}

==> tables_and_graphics/old_33_CBC_conv_comparison.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/33_CBC_conv_comparison.eps}
    % \vspace{-0.5cm}
    \caption{Convergence in the saturated heat flux value with respect to the number of points representing the velocity space. The configuration space resolution is $N_x=128$, $N_y=64$ and $N_z=24$ for both the GENE code and the GM approach. The error bars are reflects the average fluctuation amplitude around the plateau value.}
    \label{fig:33_CBC_conv_comparison}
\end{figure}
